Learning with Average Precision: Training Image Retrieval with a Listwise Loss

Image retrieval can be formulated as a ranking problem where the goal is to order database images by decreasing similarity to the query. Recent deep models for image retrieval have outperformed traditional methods by leveraging ranking-tailored loss functions, but important theoretical and practical problems remain. First, rather than directly optimizing the global ranking, they minimize an upper-bound on the essential loss, which does not necessarily result in an optimal mean average precision (mAP). Second, these methods require significant engineering efforts to work well, e.g. special pre-training and hard-negative mining. In this paper we propose instead to directly optimize the global mAP by leveraging recent advances in listwise loss formulations. Using a histogram binning approximation, the AP can be differentiated and thus employed to end-to-end learning. Compared to existing losses, the proposed method considers thousands of images simultaneously at each iteration and eliminates the need for ad hoc tricks. It also establishes a new state of the art on many standard retrieval benchmarks. Models and evaluation scripts have been made available at https://europe.naverlabs.com/Deep-Image-Retrieval/

==> algo.tex <==
\begin{algorithm}
\textbf{Inputs:} training batch $\mathcal{B}=\{(I_{1},y_{1}),\ldots,(I_{B},y_{B})\}$

\textbf{for} \emph{$i$} \textbf{in} $1..B$; \textbf{do}

~~~~compute $d_{i}\leftarrow f_{\Theta}(I_{i})$

\textbf{create} $D\leftarrow[d_{1}, \ldots, d_{B}]\in\mathbb{R}^{B\times C}$

\textbf{create} $Y\in\{0,1\}^{B\times B}$ such that $Y_{ij}=\indic[y_{i}=y_{j}]$

\textbf{$\ell\leftarrow L\left(D,Y\right)$} \textcolor{olive}{\#
compute the loss }

compute $\frac{\partial \ell}{\partial D}\in\mathbb{R}^{B\times C}$
\textcolor{olive}{\# with chain-rule}

\textbf{init} $\frac{\partial\ell}{\partial\Theta}\leftarrow 0$

\textbf{for} \emph{$i$} \textbf{in} $1..B$; \textbf{do}

~~~~compute $d_{i}\leftarrow f_{\Theta}(I_{i})$

~~~~compute $\frac{\partial d_{i}}{\partial\Theta}\leftarrow \frac{\partial }{\partial\Theta}f_{\Theta}(I_{i})$ 

~~~~accumulate $\frac{\partial\ell}{\partial\Theta}\leftarrow\frac{\partial\ell}{\partial\Theta}+\frac{\partial d_{i}}{\partial\Theta}\left(\frac{\partial\ell}{\partial D}\right)_{i}$ \textcolor{olive}{\# with chain-rule}

\textbf{update} $\Theta\leftarrow\Theta-\gamma\frac{\partial\ell}{\partial\Theta}$
\textcolor{olive}{\# optimizer step}

\caption{\label{alg:backprop}Efficient training of the gradient for arbitrary
batch size.}
\end{algorithm}


==> derivative.tex <==
In this section, we expand upon Algo. 1 from our submission to further illustrate the backpropagation process for a batch of image descriptors $D=[d_1,\dots, d_B]$ and groundtruth $Y=[Y_1, \dots,Y_B]$. Additionally, we will demonstrate the differentiability of the loss function $L$. We separate the algorithm in three stages, accordingly to Fig. 3 of our submission.

\paragraph{Stage 1.} This stage consists only of a forward pass of our network in evaluation mode, \ie no backpropagation is needed. For each image $I_i$ of the batch, its descriptor $d_i$ is computed as $d_i=f_{\Theta}(I_i)$ and the matrix $D$ is determined by the stacking of these descriptors by the rows.

\paragraph{Stage 2.} Here, we compute the loss $\ell=L(D,Y)$ given by
\begin{equation}
\ell = 1-\dfrac{1}{B}\sum_{q=1}^B\sum_{m=1}^{M} \hat{P}_{m}(d_q^\top D,Y_{q})\ \Delta \hat{r}_{m}(d_q^\top D,Y_{q}). \label{eq:ell}
\end{equation}
Since, at this stage, the backpropagation method stops at the descriptors level, our goal is to compute $\frac{\partial\ell}{\partial D}=\left(\frac{\partial \ell}{\partial d_i}\right)_{1\leq i \leq B}$.
We introduce some mathematical notations to ease the readability of this section. Let $S^q = d_q^\top D$ in $[-1,1]^B$ denote the similarities of the batch images with a
query $I_q$ in the batch, $\delta^q_m=\delta(S^q,m)$ in $[0,1]^B$ denote the soft-assignment of $S^q$ to the $m$-th bin and $\xi^q_m = \sum_{k=1}^m \delta^q_{k}$ in $\mathbb{R}^B_+$ denotes the sum of all the soft-assignments of $S^q$ up until the $m$-th bin. Moreover, $\hat{P}_m^q =\hat{P}_{m}(S^q,Y_{q})$ and $\Delta\hat{r}^q_m=\Delta \hat{r}_{m}(S^q,Y_{q})$ denote the precision and incremental recall at bin $m$ of $S^q$, respectively. These notations allow us to rewrite $\hat{P}_m^q$ and $\Delta\hat{r}^q_m$ as

\begin{align}
\hat{P}_m^q &= \dfrac{(\xi^q_m)^\top Y_q}{(\xi^q_m)^\top \text{\textbf{1}}},\\
\Delta\hat{r}^q_m &= \dfrac{(\delta^q_m)^\top Y_q}{N^q}.
\end{align}

We derivate Eq. \eqref{eq:ell} w.r.t. $d_i$ and, by applying the chain-rule, we obtain

\begingroup
\vspace{-2mm}
\addtolength{\jot}{1.0em}
\begin{align}
&\dfrac{\partial \ell}{\partial d_i} = -\dfrac{1}{B}\sum_{q=1}^B\sum_{m=1}^{M} \left(\dfrac{\partial \hat{P}_m^q}{\partial d_i}\Delta\hat{r}^q_m + \hat{P}_m^q\dfrac{\partial \Delta\hat{r}^q_m}{\partial d_i} \right) \\
&=-\dfrac{1}{B}\sum_{q=1}^B\sum_{m=1}^{M} \left( \Delta\hat{r}^q_{m}\dfrac{\partial \hat{P}_{m}^q}{\partial \xi^q_{m}}\dfrac{\partial \xi^q_{m}}{\partial S^q} + \hat{P}_{m}^q\dfrac{\partial \Delta\hat{r}^q_m}{\partial \delta^q_{m}}\dfrac{\partial \delta^q_{m}}{\partial S^q} \right)  \dfrac{\partial S^q}{\partial d_i}. \label{eq:stage2}
%&=-\dfrac{1}{B}\sum_{q=1}^B\sum_{m=1}^{M}\sum_{k=1}^m \left( \dfrac{\partial \hat{P}_{m}^q}{\partial \delta^q_{k}}\Delta\hat{r}^q_{m} + \hat{P}_{m}^q\dfrac{\partial \Delta\hat{r}^q_m}{\partial \delta^q_{k}} \right) \dfrac{\partial \delta^q_{k}}{\partial S^q} \dfrac{\partial S^q}{\partial d_i} \label{eq:stage2}
\end{align}
\endgroup
We can separately compute each of the terms of Eq. \eqref{eq:stage2}. The derivatives $\frac{\partial \delta^q_{m}}{\partial S^q}$ and $\frac{\partial \xi^q_{m}}{\partial S^q}$ in $\mathbb{R}^{B\times B}$ are defined and can be backpropagated thanks to the definition of the triangular kernel:

\begin{align}
\left(\dfrac{\partial \xi^q_{m}}{\partial S^q}\right)_{ij} &= 
\left(\sum_{k=1}^{m}\dfrac{\partial \delta^q_{k}}{\partial S^q}\right)_{ij},\label{eq:xS} \\
\left(\dfrac{\partial \delta^q_{m}}{\partial S^q}\right)_{ij} &=  -\dfrac{\text{sign}(S^q_i-b_m)}{\Delta}\indic \left[|S^q_i-b_m|\leq \Delta\right]\indic [i=j].\label{eq:dS}
\end{align}

The missing derivatives, $\frac{\partial \hat{P}^q_m}{\partial \xi^q_{m}}$ and $\frac{\partial \Delta\hat{r}^q_m}{\partial \delta^q_{m}}$ in $\mathbb{R}^{1\times B}$ and $\frac{\partial S^q}{\partial d_i}$ in $\mathbb{R}^{B\times D}$ can be expressed as follows:

\begin{align}
&\dfrac{\partial \hat{P}^q_m}{\partial \xi^q_{m}} 
= \dfrac{1}{((\xi^q_m)^\top\textbf{1})^2} (\xi^q_m)^\top \left(\textbf{1}Y_q^\top - Y_q\textbf{1}^\top \right),\label{eq:Px}\\
&\dfrac{\partial \Delta\hat{r}^q_m}{\partial \delta^q_{k}} = \dfrac{1}{N^q}Y_q^\top,\label{eq:rd}\\
&\left(\dfrac{\partial S^q}{\partial d_i}\right)_j =  d_j^\top \indic [i=q]+d_q^\top \indic [i=j] \label{eq:Sd}.
\end{align}
Finally, putting together Eqs. \eqref{eq:xS}, \eqref{eq:dS}, \eqref{eq:Px}, \eqref{eq:rd}, \eqref{eq:Sd} in Eq. \eqref{eq:stage2} proves that $L$ is differentiable and its derivative provides useful information for backpropagation.
\paragraph{Stage 3.} The goal of this stage is to compute $\frac{\partial \ell}{\partial \Theta}$. For each $i$ in $\left[1,\dots,B\right]$, $d_i=f_{\Theta}(I_i)$ and $\frac{\partial d_i}{\partial \Theta}=\frac{\partial }{\partial \Theta}f_{\Theta}(I_i)$ are computed according to the network backpropagation algorithm, and $\frac{\partial \ell}{\partial d_i}$ is obtained in stage 2. Therefore, the chain-rule give us

\begin{equation}
\dfrac{\partial \ell}{\partial \Theta} = \sum_{i=1}^B \dfrac{\partial\ell}{\partial d_i} \dfrac{\partial d_{i}}{\partial\Theta}.
\end{equation}


==> qualitative.tex <==
\def\pos{OliveGreen}
\def\neg{BrickRed}
\def\ign{YellowOrange}

In this section, we provide additional examples of queries 
and their respective top-10 result images as 
obtained by our retrieval model (referred as ``GeM (AP)'' 
in Table 1 of our submission) in the
\RParis~(Table \ref{tab:paris_medium}) and
\ROxford~(Table \ref{tab:oxford_medium})
datasets~\cite{Raden2018}. 
%
In these tables, each retrieved image is marked with a 
colored border indicating whether they belong to the 
\textcolor{\pos}{\textbf{positive}} or
\textcolor{\neg}{\textbf{negative}}
%, or \textcolor{\ign}{\textbf{ignored}}
groups of the \textit{medium} benchmark associated with these datasets
(see Section 4.1 of our submission).

\paragraph{Failure cases.}
%
At the bottom of these tables, we also list the three worst 
performing queries for each dataset. Those queries serve as
demonstrations of failure cases that can be used to indicate in 
which situations our models could be improved.
%
As it can be seen, correctly retrieving images belonging to 
these queries requires a significant level of attention to 
details, such as subtle differences in adornment statues 
(see last rows of Tables \ref{tab:paris_medium} and \ref{tab:oxford_medium}) 
or similarly looking building fa\c{c}ades seen from a short
distance (see last rows of Table~\ref{tab:oxford_medium}). 

\paragraph{Hard benchmark.}
%
We also include two other tables (Tables \ref{tab:paris_hard} and~\ref{tab:oxford_hard})
with exactly the same queries as Tables \ref{tab:paris_medium} and~\ref{tab:oxford_medium}, but
showing their evaluation under the \textit{hard} benchmark of \RParis~and \ROxford. In this protocol,
we remove easy-to-retrieve images, focusing instead on difficult cases. While 
this results in a higher amount of mistakes, our model still manages to correctly retrieve
images with varying lighting conditions (see Table \ref{tab:paris_hard}) and high 
levels of occlusion (see \nth{2} row of Table \ref{tab:paris_hard}
and \nth{5} row of Table \ref{tab:oxford_hard}).

\def\a{1.4cm}
\setlength{\tabcolsep}{0.7mm}
\renewcommand{\arraystretch}{1.5}

\newcommand{\PQ}[1]{\includegraphics[width=\linewidth,  cfbox=black 0.5mm 0mm 0mm]{figures/queries_random/RParis6K_#1.jpg}}
\newcommand{\PT}[3]{\includegraphics[width=\linewidth,  cfbox=#3    0.5mm 0mm 0mm]{figures/queries_random/RParis6K_#1_top#2.jpg}}
\newcommand{\WPQ}[1]{\includegraphics[width=\linewidth, cfbox=black 0.5mm 0mm 0mm]{figures/queries_worst/RParis6K_#1.jpg}}
\newcommand{\WPT}[3]{\includegraphics[width=\linewidth, cfbox=#3    0.5mm 0mm 0mm]{figures/queries_worst/RParis6K_#1_top#2.jpg}}



\begin{table*}[]
	\centering
	\caption{Top-10 results for 5 random queries and 3 worst-performing queries in \RParis~\cite{Raden2018}.}
	\label{tab:paris_medium}
	\begin{tabular}{m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}}
		\toprule
Query    & Top-1     & Top-2     & Top-3     & Top-4     & Top-5     & Top-6     & Top-7     & Top-8     & Top-9     & Top-10    \\
		\midrule
\multicolumn{2}{l}{\textbf{Random queries}}\\ 
\PQ{0}	 & \PT{0}{0}{\pos}  & \PT{0}{1}{\pos}  & \PT{0}{2}{\pos}  & \PT{0}{3}{\pos}  & \PT{0}{4}{\pos}  & \PT{0}{5}{\pos}  & \PT{0}{6}{\pos}  & \PT{0}{7}{\pos}   & \PT{0}{8}{\pos}  & \PT{0}{9}{\pos}  \\ 
\PQ{5}	 & \PT{5}{0}{\pos}  & \PT{5}{1}{\pos}  & \PT{5}{2}{\pos}  & \PT{5}{3}{\pos}  & \PT{5}{4}{\pos}  & \PT{5}{5}{\pos}  & \PT{5}{6}{\pos}  & \PT{5}{7}{\pos}   & \PT{5}{8}{\pos}  & \PT{5}{9}{\pos}  \\ 
\PQ{15}	 & \PT{15}{0}{\pos} & \PT{15}{1}{\pos} & \PT{15}{2}{\pos} & \PT{15}{3}{\pos} & \PT{15}{4}{\pos} & \PT{15}{5}{\pos} & \PT{15}{6}{\pos} & \PT{15}{7}{\pos}    & \PT{15}{8}{\pos} & \PT{15}{9}{\pos}   \\
\PQ{25}	 & \PT{25}{0}{\pos} & \PT{25}{1}{\pos} & \PT{25}{2}{\pos} & \PT{25}{3}{\pos} & \PT{25}{4}{\pos} & \PT{25}{5}{\pos}   & \PT{25}{6}{\pos}   & \PT{25}{7}{\pos} & \PT{25}{8}{\pos}   & \PT{25}{9}{\pos}   \\
\PQ{43}	 & \PT{43}{0}{\pos} & \PT{43}{1}{\pos} & \PT{43}{2}{\pos} & \PT{43}{3}{\pos} & \PT{43}{4}{\pos} & \PT{43}{5}{\pos} & \PT{43}{6}{\pos} & \PT{43}{7}{\pos}  & \PT{43}{8}{\pos} & \PT{43}{9}{\pos} \\
		\midrule
\multicolumn{2}{l}{\textbf{Top failure cases}}\\ 
\WPQ{66} & \WPT{66}{0}{\pos} & \WPT{66}{1}{\pos} & \WPT{66}{2}{\pos} & \WPT{66}{3}{\pos} & \WPT{66}{4}{\pos} & \WPT{66}{5}{\neg} & \WPT{66}{6}{\neg} & \WPT{66}{7}{\neg} & \WPT{66}{8}{\pos} & \WPT{66}{9}{\neg} \\
\WPQ{67} & \WPT{67}{0}{\pos} & \WPT{67}{1}{\pos} & \WPT{67}{2}{\pos} & \WPT{67}{3}{\pos} & \WPT{67}{4}{\pos} & \WPT{67}{5}{\pos} & \WPT{67}{6}{\pos} & \WPT{67}{7}{\neg} & \WPT{67}{8}{\neg} & \WPT{67}{9}{\neg} \\
\WPQ{69} & \WPT{69}{0}{\pos} & \WPT{69}{1}{\neg} & \WPT{69}{2}{\neg} & \WPT{69}{3}{\pos} & \WPT{69}{4}{\neg} & \WPT{69}{5}{\neg} & \WPT{69}{6}{\neg} & \WPT{69}{7}{\neg} & \WPT{69}{8}{\neg} & \WPT{69}{9}{\neg} \\
		\bottomrule
	\end{tabular}
\end{table*}



\renewcommand{\PQ}[1]{\includegraphics[width=\linewidth,  cfbox=black 0.5mm 0mm 0mm]{figures/queries_random/ROxford5K_#1.jpg}}
\renewcommand{\PT}[3]{\includegraphics[width=\linewidth,  cfbox=#3    0.5mm 0mm 0mm]{figures/queries_random/ROxford5K_#1_top#2.jpg}}
\renewcommand{\WPQ}[1]{\includegraphics[width=\linewidth, cfbox=black 0.5mm 0mm 0mm]{figures/queries_worst/ROxford5K_#1.jpg}}
\renewcommand{\WPT}[3]{\includegraphics[width=\linewidth, cfbox=#3    0.5mm 0mm 0mm]{figures/queries_worst/ROxford5K_#1_top#2.jpg}}


\begin{table*}[]
	\centering
	\caption{Top-10 results for 5 random queries and 3 worst-performing queries in \ROxford~\cite{Raden2018}.}
	\label{tab:oxford_medium}
	\begin{tabular}{m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}}
		\toprule
		Query   & Top-1     & Top-2     & Top-3     & Top-4     & Top-5     & Top-6     & Top-7     & Top-8     & Top-9     & Top-10    \\
		\midrule
		\multicolumn{2}{l}{\textbf{Random queries}}\\ 
		\PQ{0}	& \PT{0}{0}{\pos}  & \PT{0}{1}{\pos}  & \PT{0}{2}{\pos}  & \PT{0}{3}{\pos}  & \PT{0}{4}{\pos}  & \PT{0}{5}{\pos}  & \PT{0}{6}{\pos}  & \PT{0}{7}{\pos}  & \PT{0}{8}{\pos} & \PT{0}{9}{\pos} \\ 
		\PQ{5}	& \PT{5}{0}{\pos}  & \PT{5}{1}{\pos}  & \PT{5}{2}{\pos}  & \PT{5}{3}{\pos}  & \PT{5}{4}{\pos}  & \PT{5}{5}{\pos}  & \PT{5}{6}{\pos}  & \PT{5}{7}{\pos}  & \PT{5}{8}{\pos} & \PT{5}{9}{\pos} \\ 
		\PQ{15}	& \PT{15}{0}{\pos} & \PT{15}{1}{\pos} & \PT{15}{2}{\pos} & \PT{15}{3}{\pos} & \PT{15}{4}{\pos} & \PT{15}{5}{\pos} & \PT{15}{6}{\pos} & \PT{15}{7}{\neg} & \PT{15}{8}{\pos} & \PT{15}{9}{\neg} \\
		\PQ{33}	& \PT{33}{0}{\pos} & \PT{33}{1}{\pos} & \PT{33}{2}{\pos} & \PT{33}{3}{\pos} & \PT{33}{4}{\pos} & \PT{33}{5}{\pos} & \PT{33}{6}{\pos} & \PT{33}{7}{\pos} & \PT{33}{8}{\pos} & \PT{33}{9}{\pos} \\
		\PQ{43}	& \PT{43}{0}{\pos} & \PT{43}{1}{\pos} & \PT{43}{2}{\pos} & \PT{43}{3}{\pos} & \PT{43}{4}{\pos} & \PT{43}{5}{\pos} & \PT{43}{6}{\pos} & \PT{43}{7}{\pos} & \PT{43}{8}{\pos} & \PT{43}{9}{\pos} \\
		\midrule[0.6pt]
		\multicolumn{2}{l}{\textbf{Top failure cases}}\\ 
		\WPQ{56} & \WPT{56}{0}{\neg} & \WPT{56}{1}{\neg} & \WPT{56}{2}{\neg} & \WPT{56}{3}{\neg} & \WPT{56}{4}{\neg} & \WPT{56}{5}{\neg} & \WPT{56}{6}{\neg} & \WPT{56}{7}{\neg} & \WPT{56}{8}{\neg} & \WPT{56}{9}{\neg} \\
		\WPQ{64} & \WPT{64}{0}{\neg} & \WPT{64}{1}{\neg} & \WPT{64}{2}{\neg} & \WPT{64}{3}{\neg} & \WPT{64}{4}{\neg} & \WPT{64}{5}{\neg} & \WPT{64}{6}{\neg} & \WPT{64}{7}{\neg} & \WPT{64}{8}{\neg} & \WPT{64}{9}{\neg} \\
		\WPQ{65} & \WPT{65}{0}{\neg} & \WPT{65}{1}{\neg} & \WPT{65}{2}{\neg} & \WPT{65}{3}{\neg} & \WPT{65}{4}{\neg} & \WPT{65}{5}{\neg} & \WPT{65}{6}{\neg} & \WPT{65}{7}{\neg} & \WPT{65}{8}{\neg} & \WPT{65}{9}{\neg} \\
		\bottomrule
	\end{tabular}
\end{table*}


\renewcommand{\PQ}[1]{\includegraphics[width=\linewidth,  cfbox=black 0.5mm 0mm 0mm]{figures/queries_hard/RParis6K_#1.jpg}}
\renewcommand{\PT}[3]{\includegraphics[width=\linewidth,  cfbox=#3    0.5mm 0mm 0mm]{figures/queries_hard/RParis6K_#1_top#2.jpg}}
\renewcommand{\WPQ}[1]{\includegraphics[width=\linewidth, cfbox=black 0.5mm 0mm 0mm]{figures/queries_hard/RParis6K_#1.jpg}}
\renewcommand{\WPT}[3]{\includegraphics[width=\linewidth, cfbox=#3    0.5mm 0mm 0mm]{figures/queries_hard/RParis6K_#1_top#2.jpg}}

\begin{table*}[]
	\centering
	\caption{Top-10 results for the same queries in Table \ref{tab:paris_medium} according to 
		the \textit{hard} protocol in \RParis~\cite{Raden2018}, with \textit{easy} images removed.}
	\label{tab:paris_hard}
	\begin{tabular}{m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}}
		\toprule
		Query    & Top-1     & Top-2     & Top-3     & Top-4     & Top-5     & Top-6     & Top-7     & Top-8     & Top-9     & Top-10    \\
		\midrule
		\multicolumn{2}{l}{\textbf{Random queries}}\\ 
		\PQ{0}	 & \PT{0}{0}{\pos}  & \PT{0}{1}{\pos}  & \PT{0}{2}{\pos}  & \PT{0}{3}{\pos}  & \PT{0}{4}{\pos}  & \PT{0}{5}{\pos}  & \PT{0}{6}{\pos}  & \PT{0}{7}{\pos}   & \PT{0}{8}{\pos}  & \PT{0}{9}{\pos}  \\ 
		\PQ{5}	 & \PT{5}{0}{\pos}  & \PT{5}{1}{\pos}  & \PT{5}{2}{\pos}  & \PT{5}{3}{\pos}  & \PT{5}{4}{\pos}  & \PT{5}{5}{\pos}  & \PT{5}{6}{\pos}  & \PT{5}{7}{\pos}   & \PT{5}{8}{\pos}  & \PT{5}{9}{\pos}  \\ 
		\PQ{15}	 & \PT{15}{0}{\pos} & \PT{15}{1}{\pos} & \PT{15}{2}{\pos} & \PT{15}{3}{\pos} & \PT{15}{4}{\pos} & \PT{15}{5}{\pos} & \PT{15}{6}{\pos} & \PT{15}{7}{\neg}    & \PT{15}{8}{\neg} & \PT{15}{9}{\neg}   \\
		\PQ{25}	 & \PT{25}{0}{\pos} & \PT{25}{1}{\pos} & \PT{25}{2}{\neg} & \PT{25}{3}{\neg} & \PT{25}{4}{\neg} & \PT{25}{5}{\neg}   & \PT{25}{6}{\neg}   & \PT{25}{7}{\neg} & \PT{25}{8}{\neg}   & \PT{25}{9}{\neg}   \\
		\PQ{43}	 & \PT{43}{0}{\pos} & \PT{43}{1}{\pos} & \PT{43}{2}{\pos} & \PT{43}{3}{\pos} & \PT{43}{4}{\pos} & \PT{43}{5}{\pos} & \PT{43}{6}{\pos} & \PT{43}{7}{\pos}  & \PT{43}{8}{\pos} & \PT{43}{9}{\pos} \\
		\midrule
		\multicolumn{2}{l}{\textbf{Top failure cases}}\\ 
		\WPQ{66} & \WPT{66}{0}{\neg} & \WPT{66}{1}{\neg} & \WPT{66}{2}{\neg} & \WPT{66}{3}{\neg} & \WPT{66}{4}{\neg} & \WPT{66}{5}{\neg} & \WPT{66}{6}{\neg} & \WPT{66}{7}{\neg} & \WPT{66}{8}{\neg} & \WPT{66}{9}{\neg} \\
		\WPQ{67} & \WPT{67}{0}{\neg} & \WPT{67}{1}{\neg} & \WPT{67}{2}{\neg} & \WPT{67}{3}{\neg} & \WPT{67}{4}{\neg} & \WPT{67}{5}{\neg} & \WPT{67}{6}{\neg} & \WPT{67}{7}{\neg} & \WPT{67}{8}{\neg} & \WPT{67}{9}{\neg} \\
		\WPQ{69} & \WPT{69}{0}{\pos} & \WPT{69}{1}{\neg} & \WPT{69}{2}{\neg} & \WPT{69}{3}{\pos} & \WPT{69}{4}{\neg} & \WPT{69}{5}{\neg} & \WPT{69}{6}{\neg} & \WPT{69}{7}{\neg} & \WPT{69}{8}{\neg} & \WPT{69}{9}{\neg} \\
		\bottomrule
	\end{tabular}
\end{table*}



\renewcommand{\PQ}[1]{\includegraphics[width=\linewidth,  cfbox=black 0.5mm 0mm 0mm]{figures/queries_hard/ROxford5K_#1.jpg}}
\renewcommand{\PT}[3]{\includegraphics[width=\linewidth,  cfbox=#3    0.5mm 0mm 0mm]{figures/queries_hard/ROxford5K_#1_top#2.jpg}}
\renewcommand{\WPQ}[1]{\includegraphics[width=\linewidth, cfbox=black 0.5mm 0mm 0mm]{figures/queries_hard/ROxford5K_#1.jpg}}
\renewcommand{\WPT}[3]{\includegraphics[width=\linewidth, cfbox=#3    0.5mm 0mm 0mm]{figures/queries_hard/ROxford5K_#1_top#2.jpg}}


\begin{table*}[]
	\centering
	\caption{Top-10 results for the same queries in Table \ref{tab:oxford_medium} according to 
		the \textit{hard} protocol in \ROxford~\cite{Raden2018}, with \textit{easy} images removed.}
	\label{tab:oxford_hard}
	\begin{tabular}{m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}m{\a}}
		\toprule
		Query   & Top-1     & Top-2     & Top-3     & Top-4     & Top-5     & Top-6     & Top-7     & Top-8     & Top-9     & Top-10    \\
		\midrule
		\multicolumn{2}{l}{\textbf{Random queries}}\\ 
		\PQ{0}	& \PT{0}{0}{\pos}  & \PT{0}{1}{\pos}  & \PT{0}{2}{\neg}  & \PT{0}{3}{\neg}  & \PT{0}{4}{\neg}  & \PT{0}{5}{\neg}  & \PT{0}{6}{\neg}  & \PT{0}{7}{\neg}   & \PT{0}{8}{\pos}  & \PT{0}{9}{\pos}  \\ 
		\PQ{5}	& \PT{5}{0}{\pos}  & \PT{5}{1}{\neg}  & \PT{5}{2}{\neg}  & \PT{5}{3}{\neg}  & \PT{5}{4}{\pos}  & \PT{5}{5}{\neg}  & \PT{5}{6}{\neg}  & \PT{5}{7}{\neg}   & \PT{5}{8}{\neg}  & \PT{5}{9}{\neg}  \\ 
		\PQ{15}	& \PT{15}{0}{\neg} & \PT{15}{1}{\neg} & \PT{15}{2}{\neg} & \PT{15}{3}{\neg} & \PT{15}{4}{\neg} & \PT{15}{5}{\neg} & \PT{15}{6}{\neg} & \PT{15}{7}{\neg}    & \PT{15}{8}{\neg} & \PT{15}{9}{\neg}   \\
		\PQ{33}	& \PT{33}{0}{\pos} & \PT{33}{1}{\neg} & \PT{33}{2}{\neg} & \PT{33}{3}{\neg} & \PT{33}{4}{\pos} & \PT{33}{5}{\pos} & \PT{33}{6}{\neg} & \PT{33}{7}{\neg} & \PT{33}{8}{\neg} & \PT{33}{9}{\neg} \\
		\PQ{43}	& \PT{43}{0}{\pos} & \PT{43}{1}{\pos} & \PT{43}{2}{\pos} & \PT{43}{3}{\pos} & \PT{43}{4}{\neg} & \PT{43}{5}{\pos} & \PT{43}{6}{\pos} & \PT{43}{7}{\pos} & \PT{43}{8}{\pos} & \PT{43}{9}{\pos} \\
		\midrule[0.6pt]
		\multicolumn{2}{l}{\textbf{Top failure cases}}\\ 
		\WPQ{56} & \WPT{56}{0}{\neg} & \WPT{56}{1}{\neg} & \WPT{56}{2}{\neg} & \WPT{56}{3}{\neg} & \WPT{56}{4}{\neg} & \WPT{56}{5}{\neg} & \WPT{56}{6}{\neg} & \WPT{56}{7}{\neg} & \WPT{56}{8}{\neg} & \WPT{56}{9}{\neg} \\
		\WPQ{64} & \WPT{64}{0}{\neg} & \WPT{64}{1}{\neg} & \WPT{64}{2}{\neg} & \WPT{64}{3}{\neg} & \WPT{64}{4}{\neg} & \WPT{64}{5}{\neg} & \WPT{64}{6}{\neg} & \WPT{64}{7}{\neg} & \WPT{64}{8}{\neg} & \WPT{64}{9}{\neg} \\
		\WPQ{65} & \WPT{65}{0}{\neg} & \WPT{65}{1}{\neg} & \WPT{65}{2}{\neg} & \WPT{65}{3}{\neg} & \WPT{65}{4}{\neg} & \WPT{65}{5}{\neg} & \WPT{65}{6}{\neg} & \WPT{65}{7}{\neg} & \WPT{65}{8}{\neg} & \WPT{65}{9}{\neg} \\
		\bottomrule
	\end{tabular}
\end{table*}




==> sec_backprop.tex <==
\subsection{Backpropagation of AP loss and minibatch sampling}

%Training a neural network for multiclass image retrieval with AP loss can lead to memory issues for big batches.
%In this section, we discuss the our solution to the backpropagation of the AP loss for big batch sizes.

The experiments of He et al. \cite{} in patch retrieval reinforce the idea that we can obtain better performances with global ranking losses by increasing the batch size in train time. However, global descriptors for image retrieval are very sensitive to image resolution. The combination of high resolution images and large batch size results in memory issues. More specifically, for a batch size $B$ too large, we can not store and backpropagate gradients through very deep architectures such as ResNet-101. Conversely, while optimizing the AP loss of a given query, only a few images (positives and hard negatives) are interesting to our loss, since most of the distractors are trivial negatives. In this section, we discuss our proposed modifications to the optimization scheme of the AP loss in order to address this issue.

Let $b$ denote a batch-size compatible to the memory limitations of our architecture. In practice, $b$ is too small to obtain good performances with AP loss.
We propose below an optimization scheme that allow us to backpropagate the AP loss through \textit{minibatches} of size $b$ while maximizing the AP loss in a batch of size $B$.

\begin{enumerate}
	\item Sample $B$ images $\{I_i\}_{1\leq i\leq B}$ and its groundtruth $G=\{
	\textbf{1}_{y(I_i)=y(I_j)}\}_{1\leq i,j \leq B}$ from the training set, while guaranteeing that every class present in the batch has at least two images.
	\item Compute static versions of the embeddings of $D=\{f_{\theta}(I_i)\}_{1\leq i\leq B}$ of the batch and the similarity matrix $S=\{s_{ij}\}_{1\leq i,j \leq B}$, which we call $D^{sta}$ and $S^{sta}$, respectively.
	\item Batch reshuffling of images and groundtruth.
	\item For a minibatch $\{I_k\}_{i\leq k \leq i+b}$, $b \in \{1, b+1, \dots, B+1-b\}$:
	\begin{enumerate}
		\item Compute dynamic embeddings $D_{dyn}^i=\{f_{\theta}(I_k)\}_{i\leq k\leq i+b}$ and dynamic similarity matrix $S_{dyn}^i$, given by:
		
		\item Compute and backpropagate the \texit{APLoss}$(S_{dyn}^i,G)$
	\end{enumerate}
	
\end{enumerate}
 
In the above algorithm, we distinguish between dynamic and static variables as being attached to neural networks gradients or not, respectively.

\paragraph{Batch reshuffling}
The proposed algo/heuristic/scheme (?) does not backpropagates the same gradient as an hypothetical backwards pass of the batch of size $B$. Indeed, this scheme proposes an asymmetrical approximation: we correctly compute the gradient for $s_{ij}$ if images $I_i$ and $I_j$ are in the same minibatch and only approximate it if they are not. While it means that we only approximate the gradient of most entries of the similarity matrix $S$, we notice that this approximation is good enough if $s_{ij}$ is small and $I_i, \ I_j$ do not correspond to the same class, \ie $I_i, \ I_j$ are trivial negatives of each other.

TL;DR: we do a label-based minibatching of our big batch. Or a one-dimension projection to reshuffle out batch such that close embeddings are in the same minibatch.

1. We guarantee a bigger number queries with non-zero gradients if all classes are represented in each batch.

2. By clustering our big batch by class labels, we can accelerate the convergence of the AP of this class.

3. by including neighboring embeddings in the same minibatch, we prioritize the gradient of the most important impactful points to the AP.
